Learning Visual Robotic Control Efficiently with Contrastive Pre-training and Data Augmentation

Recent advances in unsupervised representation learning significantly improved the sample efficiency of training Reinforcement Learning policies in simulated environments. However, similar gains have not yet been seen for real-robot reinforcement learning. In this work, we focus on enabling data-efficient real-robot learning from pixels. We present Contrastive Pre-training and Data Augmentation for Efficient Robotic Learning (CoDER), a method that utilizes data augmentation and unsupervised learning to achieve sample-efficient training of real-robot arm policies from sparse rewards. While contrastive pre-training, data augmentation, demonstrations, and reinforcement learning are alone insufficient for efficient learning, our main contribution is showing that the combination of these disparate techniques results in a simple yet data-efficient method. We show that, given only 10 demonstrations, a single robotic arm can learn sparse-reward manipulation policies from pixels, such as reaching, picking, moving, pulling a large object, flipping a switch, and opening a drawer in just 30 minutes of mean real-world training time. We include videos and code on the project website: https://sites.google.com/view/efficient-robotic-manipulation/home

==> content/approach2.tex <==


\section{Method}
\begin{wrapfigure}{r}{0.65\textwidth}
  \centering
  \begin{subfigure}{.3\linewidth}
    \centering\includegraphics[width=.9\linewidth]{figures/FetchReach-v1.png}
    \subcaption{{\small FetchReach}}
  \end{subfigure}
  \begin{subfigure}{.3\linewidth}
    \centering\includegraphics[width=.9\linewidth]{figures/FetchPickAndPlace-v1.png}
    \subcaption{{\ssmall FetchPickAndPlace}}
  \end{subfigure}
  \begin{subfigure}{.3\linewidth}
    \centering\includegraphics[width=.9\linewidth]{figures/FetchPush-v1.png}
    \caption{{\small FetchPush}}
  \end{subfigure}
  \label{fig:fetch_envs}
  \vspace{1mm}
  \caption{{\small
  Simulated environments from OpenAI gym~\cite{openaigym} used in addition to our real robot experiments. We use the Fetch Gym Suite to investigate the core components of \coder.}
%   We utilize (left to right) FetchReach, FetchPickAndPlace, and FetchPush from the Fetch Gym Suite.
%   Shown are sample observations from the third person camera, as well as 
%   \textbf{FetchReach}: The gripper must move to the target location, shown in red. \textbf{FetchPickAndPlace}: The gripper must pick the object, and place it on the goal. \textbf{FetchPush}: The gripper is used to push the object to the goal.
  %In addition to the real robot experiments, we also include simulated experiments to investigate the core components of the FERM method. We utilize the Fetch Gym suite of environments \cite{openaigym}, which includes the reach, push, and pick-and-place tasks.
  }
  \vspace{5mm}
\end{wrapfigure}

Our proposed framework, shown in Figure~\ref{fig:architecture}, combines demonstrations, unsupervised pre-training, and off-policy model-free RL with data augmentation into one holistic Framework. \coder has three distinct steps -- (i) minimal collection of demonstrations (ii) encoder initialization with unsupervised pre-training and (iii) online policy learning through RL with augmented data
-- which we describe in detail below.

{\bf Minimal Collection of Demonstrations:} We initialize the replay buffer with a small number of expert demonstrations (we found $10$ to be sufficient) for each task. Demonstrations are collected with a joystick controller, shown in Figure~\ref{fig:teaser}. Our goal is to minimize the total time required to acquire a skill for an RL agent, including both policy training as well as time required to collect demonstrations. While collecting a larger number of demonstrations certainly improves training speed, we find 10 demonstrations is already sufficient to learn skills quickly (see Fig.~\ref{fig:abalation_demo}). For real world experiments, collecting $10$ expert demonstrations can be done within $10$ minutes
% (see Table~\ref{tab:robot_time_SR}), 
which includes the time needed to reset the environment after every demonstration. 

{\bf Unsupervised Encoder Pre-training:} After initializing the replay buffer with 10 demonstrations, we pre-train the convolutional encoder with instance-based contrastive learning, using stochastic random crop \cite{laskin2020curl} to generate query-key pairs. 
The key encoder is an exponentially moving average of the query encoder \cite{kaiming2019moco}, and the similarity measure between query-key pairs is the bi-linear inner product \cite{oord2018representation} shown in Equation~\ref{eq:infonce}. 
Note that the bi-linear inner product is only used to pre-train the encoder. 
After pre-training, the weight matrix in the bi-linear measure is discarded. 

{\bf Reinforcement Learning with Augmented Data:} After pre-training the convolutional encoder on offline demonstration data, we train a SAC \cite{haarnoja2018soft} agent with data augmentation \cite{laskin_lee2020rad} as the robot interacts with the environment. Since the replay buffer was initialized with demonstrations and SAC is an off-policy RL algorithm, during each minibatch update the agent receives a mix of demonstration observations and observations collected during training when performing gradient updates. The image augmentation used during training is random crop -- the same augmentation used during contrastive pre-training. 

%These three steps -- collecting 10 demonstrations, contrastive pre-training of the encoder, and off-policy RL with data augmentation -- comprise our framework for efficient robotic manipulation. \pz{Might be redundant.}


==> content/baselines.tex <==
\subsection{Qualitative Analysis \& Baselines}

\begin{wrapfigure}{r}{0.35\textwidth}
    \vspace{-2mm}
    % \centering
    \includegraphics[height=3.3cm, trim={20px 0px 20px 10px}, clip]{figures/baselines/real_robot_bc2.png}
    % \includegraphics[height=3.2cm]{figures/baselines/pickup.png}
    % \includegraphics[height=3.2cm, trim={10px 0px 40px 20px}, clip]{figures/ablation_warmup_pnp.png}
    % \includegraphics[height=3.2cm, trim={10px 0px 40px 20px}, clip]{figures/ablation_warmup_pick.png}
%   \caption{Behavior cloning behavior on the Light Switch and Pickup task. Using the same demonstrations as our method, behavior cloning has limited capabilities due to low amounts of demonstrations.}
% \label{fig:baselines}
% \vspace{-6mm}
    % \vspace{5pt}
    % \includegraphics[height=3.2cm, trim={10px 0px 40px 20px}, clip]{figures/baselines/reach_bc.png}
    % \includegraphics[height=3.2cm, trim={10px 0px 40px 20px}, clip]{figures/baselines/pnp_bc.png}
    % \includegraphics[height=3.2cm, trim={10px 0px 40px 20px}, clip]{figures/ablation_warmup_pnp.png}
    % \includegraphics[height=3.2cm, trim={10px 0px 40px 20px}, clip]{figures/ablation_warmup_pick.png}
%   \caption{In simulation, the Behavior cloning baseline is only able to recover a sub-optimal policy for the Reach task.}

    \caption{Reported are the success rates on the Light Switch and Pickup task from Figure 5.}
    % \ferm is able to complete the task on every evaluation.}
\label{fig:baselines}
\vspace{-3mm}
\end{wrapfigure}

For our real world experiments, we qualitatively examine the policies learnt using \ferm versus behavior cloning from the same 10 demonstrations on a random goal (pickup), and a fixed goal task (switch). 
Videos of the policies are on the project website\footnote{\url{https://sites.google.com/view/efficient-visual-robotics}}, as well as the video in the Supplementary Materials.
% For the light switch task, even though the light switch remained stationary during training and demonstrations, the \ferm policy generalizes, and is able to complete the task even when the switch is moved to a never before seen location. 

We found that behavior cloning was able to complete the task around half of the time (17/30 trials) at the same position,
as the policy learned to memorize the steps necessary to flip the switch at the specified position. The most frequent failure mode occurred when the policy did performed the movement to flip the switch, but missed the actual switch. When the switch was moved from the training and demonstration location, this failure was inevitable every time. 
In contrast, the \ferm policy generalizes, and is able to complete the task even when the switch is moved to a never before seen location.

For the Pickup task, the policy trained with \ferm has intrinsic robustness to perturbation and generalization.
When the block is poked with a stick, the policy is able to recover even when the block is poked out from the gripper.
As well, the policy generalizes to pick up similarly colored blocks with different shapes.

The pickup policy learnt through behavior cloning was unable to locate the block at all, due to the low amount of demonstrations.
Even with lucky resets near the block, the policy is not robust to interactions with the block and fails to pick the block up.

==> content/conclusion.tex <==
\section{Conclusion and Future Work}
% Connect to insights from approach and results

We present \fermNoSpace, a framework that combines demonstrations, unsupervised learning, and RL, to efficiently learn complex tasks in the real world.
Using image input, our method is able to successfully solve a diverse set of tasks, all using the same hyperparameters, and from sparse reward.
Due to the limited amount of supervision required, our work presents exciting avenues for applying RL to real robots in a quick and efficient manner.


==> content/implementation_details.tex <==
\subsection{Implementation Details}

Listed below is the hyperparameter table used in our real world and simulated environments.
\begin{table}[h]
\caption{Training Hyperparameters}
\label{table:hyperparameters}
\vskip 0.15in
\begin{center}
\begin{tabular}{ll}
\toprule
\textbf{Hyperparameter} & \textbf{Value}  \\
\bottomrule 
\toprule 
\textbf{\ferm}  & \\
\midrule  
Data Augmentation & Random Crop \\
    \: Crop Size & $84$x$84$ \\
Environment Observation Size  \qquad \qquad \qquad & $ 100$ x $100$ \\
Environment Steps & $200$k (Sim), $3000$ (Real World) \\
Environment Horizon & $50$ (Sim), $30$ (Real World) \\
Batch size & $128$ \\
\textbf{Critic} & \\
    \: LR & 1e-3 \\
    \: $\beta$ & $0.9$ \\
    \: $\tau$ & $0.01$ \\
    \: Target Update Frequency & $2$ \\
\textbf{Actor} & \\
    \: LR & 1e-3 \\
    \: $\beta$ & 0.5 \\ 
    \: Target Update Frequency & $2$ \\
\textbf{Critic \& Actor Architecture} & \\
    \: Hidden Layer Size & 1024 \\
    \: \# Hidden Layers & $2$ \\
    \: Activation & ReLU \\
    \: \textbf{Encoder} & \\
        \quad Conv Layers & $4$ \\
        \quad \# Filters & $32$ \\
        \quad Kernel Size & $3$ \\
        \quad Stride & $(2, 1, 1, 1)$ \\
        \quad Feature Dimension & 50 \\
        \quad Layer Norm & $\epsilon=$1e-5 \\
        \quad LR & 1e-3 \\
        \quad $\tau$ & 0.05 \\

Discount $\gamma$ & $0.99$ \\

Updates per Environment Step & $5$ (Sim), $10$ (Real World) \\
Optimizer & Adam($\beta_1=0.9$, $\beta_2=0.999$, LR=$1\text{e-}3$) \\
\bottomrule 
\toprule 
\textbf{RAD baseline} & \\
\midrule 
Initial Random Steps & $1000$ (Sim), $150$ (Real World) \\
\bottomrule 
\toprule 
\textbf{BC baseline} & \\
\midrule 
Epochs & $200$ \\
% Batch size & $128$ \\
Optimizer & Adam($\beta_1=0.9$, $\beta_2=0.999$, LR=$1\text{e-}3$) \\
\bottomrule 
\end{tabular}
\end{center}
\vskip -0.1in
\end{table}


==> content/real_robot.tex <==
\subsection{Manipulation with sparse reward.}
Results to put in the paper:
\begin{enumerate}
    \item Table of 4 tasks. Show task difficulty, time of first encounter and time of reliable completion.
\end{enumerate}

==> content/robotic_results_table.tex <==
\begin{table}[h!]
\begin{center}
% \setlength{\tabcolsep}{10pt}
\newcommand{\rescellwidth}{1.55cm} %use 1.15 for multiline but thinner cell look
\begin{tabular}{|l|>{\raggedleft\hspace{0pt}}p{\rescellwidth}|>{\raggedleft\hspace{0pt}}p{\rescellwidth}|>{\raggedleft\hspace{0pt}}p{\rescellwidth}|>{\raggedleft\hspace{0pt}}p{\rescellwidth}|>{\raggedleft\hspace{0pt}}p{\rescellwidth}|>{\raggedleft\hspace{0pt}}p{\rescellwidth}|}
\hline
  &&&&&& \tabularnewline
%   \multirow{1}{0.8cm}{Tasks} & 
%   \multirow[r]{1}{.45cm}{}{Reach} &
%   \multirow[r]{1}{.45cm}{}{Pickup} &
%   \multirow[r]{1}{.45cm}{}{Move} & 
%   \multirow[r]{1}{.45cm}{}{Pull} &
%   \multirow[r]{1}{.45cm}{}{Switch} &
%   \multirow[l]{1}{.45cm}{}{Drawer} \\
    Tasks & Reach & Pickup & Move & Pull & Light Switch & Drawer Open \tabularnewline
%   &&&& \\
\hline
% \tabularnewline
\hline
  Time to record Demonstrations (min) & \textless 10:00  & \textless 10:00 & \textless 10:00 & \textless 10:00 & \textless 10:00 & \textless 10:00 \tabularnewline 
  \# Expert demonstrations & 10 & 10 & 10 & 10 & 10 & 10 \tabularnewline
  \hline 
\hline 
 Time to First Success (mm:ss) & 3:05 & 15:00 & 33:00 & 05:12 & 05:01 & 5:56 \tabularnewline
% \hline
 \# Episodes to First Success  & 6 & 30 & 40 & 5 & 6 & 7 \tabularnewline
% \hline
 Time to Optimal Policy (mm:ss) & 15:00  & 26:00 & 46:00 & 29:10 & 16:05 & 20:21 \tabularnewline
% \hline
 \# Episodes to Optimal Policy & 20 & 60 & 80 & 45 & 20 & 25 \tabularnewline
\hline \hline 
 Number of Successes for Eval (  /30) & 30 & 30 & 26 & 28 & 30 & 30 \tabularnewline
 Success Rate for Eval (\%) & 100 & 100 & 86.7 & 93.3 & 100 & 100 \tabularnewline

 \hline 
 
\end{tabular}
\caption{The speed at which our agents learn to complete the tasks. 
Listed above are the to demonstration collection times, as well as the time at which the policy first achieves a success, and when an optimal policy is learnt. 
The optimal policy is then used to evaluate for 30 episodes, and the number of successes and the converted success rates are shown. 
Our method starts to complete the tasks in around 30 minutes of training, and as little as 3 minutes for simple tasks such as Reach.
}
\label{tab:robot_time_SR}

\end{center}
\vspace{-6mm}

\end{table}

==> content/task_description.tex <==
\subsection{Task Description}
\label{appendix:tasks}
\label{sec:task_details_short}

For all of our real robot tasks, the reward function is the same as the discrete reward in Fetch suite, with $0$ when the task is in a completion state, and $-1$ everywhere else. 
% Since policy evaluation requires a task success function (usually done via human labeling), using this function as reward signal is feasible for how fast \ferm trains.
By design, our experiments are easy to reset at completion states, by simple hard-coded procedures.
Our assumptions allow \ferm to simply run with very little supervision, where the only human supervision is the 10 collected demonstrations.
% To speed up learning on the real robot, the episode length is shortened to 30 steps, rather than the default 50 in the Fetch suite. The normalized reward is computed by adding the episode length to the reward, and dividing by the episode length.

\begin{enumerate}
    \item \textbf{Reach}:
    The Robot must move to the block location. We consider a success when the gripper camera view has the block in its center. 
    The gripper is constrained to be unable to reach low enough to interact with the block. The gripper aperture is locked to a set position.
    During training, we fix the block location, however the demonstrations include random block locations.
    The arm is reset to a random location after every episode.
    \item \textbf{Pickup}:
    Success is declared if the robot picks the block up a specified height (70mm) above the work surface.
    At the end of each episode, if the gripper is around the block, it will reset the block to a random position, as well, resetting the gripper to a random location.
    \item \textbf{Move}:
    An episode is deemed successful when the block is moved to the center, onto the goal. Specifically, reward is given when the goal and the block are close while both visible from the griper camera.
    This task is especially difficult, as the block can be anywhere relative to the goal, so the system must understand to move the block in many directions, rather than a generic direction.
    As with Pickup, the block is reset at the end of each episode if the gripper can close and pick the block to a random location.
    \item \textbf{Pull}:
    The gripper aperture is locked at a set position.
    Without gripping onto the sponge, the robot must pull the sponge to an area around its base.
    At the end of each successful episode, the sponge is moved to a new random position.
    \item \textbf{Light switch}:
    A light switch panel is fixed to the work surface, and a blue LED lights up when the switch is flipped on.
    The gripper aperture is locked at a set position.
    Reward is given when blue light is visible from the gripper camera. At the end of each episode, a hard-coded reset procedure is executed to turn off the light. 
    \item \textbf{Drawer open}:
    The drawer is fixed to the work surface. The robot must grab onto the handle to pull open the drawer. Success is declared when the handle is visible from the gripper camera while the gripper position corresponds to the drawer being open. The drawer is closed by a hard-coded reset procedure at the end of each episode.
    
\end{enumerate}

For Reach, Light switch, and Drawer open tasks, the goal is fixed, and so the reset is hard-coded. 
For Pickup and Move, the block is only reset to a random location when the gripper is gripping the block, and for Pull, the sponge is only reset upon successfully pulling the sponge to the base of the robot.
% Although we used resets, the resets are only used upon success (near-success for Pickup and Move). 
% Our reward function is a less constrictive version than other RL methods, such as dense rewards, or Reward Sketching. 

==> content/task_description_short.tex <==
\section{Real Robot Task Details}

\label{sec:task_details_short}

In all the tasks, the gripper is reset to a random location at the beginning of an episode. The sparse reward is $0$ on task completion, otherwise $-1$.

\textbf{Reach}: the robot must move its gripper to the block location. We consider a success when the gripper camera view has the block in its center.
\textbf{Pickup}: Task is done if the robot picks up the block beyond a specified height (70mm) above the work surface. 
\textbf{Move}: an episode is deemed successful when the block is moved onto a red goal pad. This task is especially difficult, as the block can be anywhere relative to the goal.
\textbf{Pull}: the gripper aperture is locked at a set position. Without gripping onto the sponge, the robot must pull the sponge to an area around its base. 
\textbf{Light switch}: a switch panel is fixed to the work surface, controlling a blue LED. The gripper aperture is locked. Reward is given when blue light is visible from the gripper camera.
\textbf{Drawer open}: the robot must grab onto the handle to pull open the drawer. Success is declared when the drawer is opened beyond a set distance (100mm).

For \textit{pickup} and \textit{move}, if the gripper is around the block at the end of an episode, it resets the block to a random position. For \textit{pull}, the sponge is moved to a new random position at the end of each successful episode.


==> hyperparameters.tex <==
% \begin{table}[!h]
% \begin{center}
% \begin{tabular}{|l|c|}
% \hline 
% SAC hyperparameters & \\
% Encoder $\tau$ & 0.05 \\  
% Q function $\tau$ & 0.01 \\
% $\log{\sigma}$ & $\in [-10, 2]$ \\
% $|\mathcal{B}|$ & 1e6 \\
% \hline 

% \end{tabular}
% \end{center}
% \label{tab:hyperparams}
% \end{table}
\subsection{Hyperparameters}
Our RAD SAC hyperparameters are mostly the same as in \cite{laskin_lee2020rad}. The details are reproduced in the table below.

\begin{table}[h]
\caption{Hyperparameters used for the 6 tasks and simulated ablations investigated in this work.}

\label{table:hyperparameters}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{ll}
\toprule
\textbf{Hyperparameter} & \textbf{Value}  \\
\midrule
Random crop    & True  \\ 
Raw Observation     & $(100,100)$  \\ 
Observation after crop    & $(84,84)$  \\ 
Replay buffer size    & $100000$ \\ 
Initial steps    & $1000$ for sim, $0$ for xArm \\ 
Stacked frames    & $1$  \\ 
Action repeat    & $1$  \\
Hidden units (MLP)    & $1024$  \\ 
Evaluation episodes    & $100$, only in sim \\ 
Optimizer    & Adam  \\ 
$(\beta_1,\beta_2) \rightarrow (f_\theta, \pi_\psi, Q_\phi)$   & $(.9,.999)$  \\
$(\beta_1,\beta_2) \rightarrow (\alpha)$   & $(.5,.999)$  \\
Learning rate $(f_\theta, \pi_\psi, Q_\phi)$   & $1e-4$ \\

Batch Size    & $128$  \\ 
$Q$ function EMA $\tau$ & $0.01$ \\
Critic target update freq & $2$ \\
Convolutional layers & $4$ \\
Number of filters & $32$ \\
Non-linearity & ReLU \\
Encoder EMA $\tau$ & $0.05$ \\
Latent dimension & $50$ \\
Discount $\gamma$ & $.99$ \\
Initial temperature & $0.1$ \\


\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\subsection{Experiment Details}
Following CURL, we re-use the key encoder as the encoder for the target networks used in the SAC algorithm. 
The same $\tau$ coefficient used for the pre-training is used during training to EMA the target weights. 

\subsubsection{Simulation Robot}
For our robot in sim, we modify the Fetch environments \cite{fetch2016} to include multi-camera setup. 
The demonstrations for the sparse reward tasks are collected by rolling out a state-input expert policy, which was trained with SAC on dense reward.
